GANalyze: Toward Visual Definitions of Cognitive Image Properties

We introduce a framework that uses Generative Adversarial Networks (GANs) to study cognitive properties like memorability, aesthetics, and emotional valence. These attributes are of interest because we do not have a concrete visual definition of what they entail. What does it look like for a dog to be more or less memorable? GANs allow us to generate a manifold of natural-looking images with fine-grained differences in their visual attributes. By navigating this manifold in directions that increase memorability, we can visualize what it looks like for a particular generated image to become more or less memorable. The resulting ``visual definitions" surface image properties (like ``object size") that may underlie memorability. Through behavioral experiments, we verify that our method indeed discovers image manipulations that causally affect human memory performance. We further demonstrate that the same framework can be used to analyze image aesthetics and emotional valence. Visit the GANalyze website at http://ganalyze.csail.mit.edu/.

==> GANalyze preprint/latex/teaser2.tex <==
%\begin{multicols}{2}
\begin{figure}[h!]
\begin{minipage}{\textwidth}
	\centering
	\vspace{0.0in}
%\includegraphics[width=\textwidth]{latex/teaser.jpg}

\includegraphics[width=480pt]{latex/teaser2_figure.pdf}
%\hspace{10pt}
%\includegraphics[width=240pt]{latex/examples_teaser_1.pdf}
\caption{\textbf{Visualizations produced by the proposed GANalyze framework}. The middle columns represent generated images serving as the original seed. The originals are then modified to be characterized more (right) or less (left) by a given property of interest (memorability, aesthetics, or emotional valence). The images' respective property scores are presented in their top left corner.}

\label{fig:teaser}
\end{minipage}
%\vspace{-1.3in}

\end{figure} 

%\end{multicols}
